TERA: A Simulation Environment for Terrain Excavation Robot Autonomy

Developing excavation autonomy is challenging given the environments where excavators operate, the complexity of physical interaction and the degrees of freedom of operation of the excavator itself. Simulation is a useful tool to build parts of the autonomy without the complexity of experimentation. Traditional excavator simulators are geared towards high fidelity interactions between the joints or between the terrain but do not incorporate other challenges such as perception required for end to end autonomy. A complete simulator should be capable of supporting real time operation while providing high fidelity simulation of the excavator(s), the environment, and their interaction. In this paper we present TERA (Terrain Excavation Robot Autonomy), a simulator geared towards autonomous excavator applications based on Unity3D and AGX that provides the extensibility and scalability required to study full autonomy. It provides the ability to configure the excavator and the environment per the user requirements. We also demonstrate realistic dynamics by incorporating a time-varying model that introduces variations in the system's responses. The simulator is then evaluated with different scenarios such as track deformation, velocities on different terrains, similarity of the system with the real excavator and the overall path error to show the capabilities of the simulation.

==> tables/limits.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
\centering
\begin{tabular}{@{}c|c|cc@{}}
\toprule
Link   & Mass (kg) & \multicolumn{2}{c}{Joint Limits (rads)}  \\ \midrule
       &           & \multicolumn{1}{c|}{Min}   & Max  \\ \midrule
Bucket & 132.71    & \multicolumn{1}{c|}{-1.82} & 0.87 \\
Arm    & 265.34    & \multicolumn{1}{c|}{-0.4}  & 1.8  \\
Boom   & 694.17    & \multicolumn{1}{c|}{-1.57} & 1.57 \\
Swing  & 98.14     & \multicolumn{1}{c|}{-1.57} & 1.57 \\
Plow   & 147.01    & \multicolumn{1}{c|}{0}     & 0.52 \\ \bottomrule
\end{tabular}
\caption{Link and Joint Properties of the Manipulation System}
\label{table:limits}
\end{table}

==> tables/msg.tex <==

\begin{figure}
    \begin{minted}[
    gobble=4,
    frame=single,
  ]{yaml}
    std_msgs/Header header  
    float32 mslewcmd
    float32 mboomcmd
    float32 mbucketcmd
    float32 marmcmd
    float32 mlefttravelcmd
    float32 mrighttravelcmd
    float32 mbladecmd_a
    float32 mswingcmd_a
    float32 mthumbcmd_a
    float32 mbladecmd_b
    float32 mswingcmd_b
    float32 mthumbcmd_b
    float32 mhydraulic
    float32 mhorn
    float32 menableautonav
    \end{minted}
    \caption{DeltaCAN message}
    \label{fig:deltacan}
\end{figure}

